Measuring the Kapitza Resistance between a Passivated Semiconductor and Liquid Helium

In this paper, we describe an experimental investigation into the effect of passivation layer thickness on heat dissipation between a quartz substrate and liquid helium. We have observed that by depositing SiN from 0 to 240 nm, the Kapitza resistance increases by 0.0365 m^2.K/W per nanometer more than for an unpassivated semiconductor. We hypothesize that this increase in Kapitza resistance represents an additional barrier to the cooling of semiconductor devices in liquid helium.

==> note.tex <==
|%Another important consideration in understanding heat transfer at the interface is the diffuse mismatch theory \cite{b211} which is related to  phonon scattering at the interface due to their wavelength. %The effect of phonon wavelength on Kapitza resistance is such that larger wavelengths promote more efficient heat transfer.\\
%When the phonon wavelength is much larger than the characteristic dimensions of the interface, such as the inter-atomic spacing or the thickness of the interface region, the phonons tend to propagate relatively freely across the interface. This results in a lower Kapitza resistance as the phonons can efficiently transfer heat. However, smaller wavelengths introduce greater resistance. When the phonon wavelength becomes comparable to or smaller than the characteristic dimensions of the interface, phonon scattering and reflection at the interface become more significant. This leads to increased resistance to phonon transport and, consequently, a higher Kapitza resistance \cite{b20},\cite{b22,b233,b234}. \\ %We estimate that this passivation layer acts as a reflective coating layer for phonons, and characterizing the passivation layer thickness to achieve minimum Kapitza resistance leads to better heat dispersion. The results can then be applied to low-noise electronics such as  HEMT-based amplifiers to study noise behavior.\\ 
%Further, Considering  \cite{b23} and \cite{b24},   
%table \ref{tab:PhononWavelength} provides the range of dominant phonon wavelength at different temperatures for the applied materials in this experiment.
%\begin{table}[h!]
%\caption{Dominant phonon wavelength}
%\label{tab:PhononWavelength}
%\centering
%\renewcommand{\arraystretch}{1.5}
%\begin{tabular}{lcc}
%\hline
%Material & \multicolumn{2}{c}{Wavelength (nm)} \\

 %& 300K&77K \\
%\hline
%\hline
%Au &0.152-0.226&0.89-72.6 \\
%SiN &0.314-66.78 &0.1430- \\
%\hline
%\end{tabular}
%\end{table}%


%It can be anticipated that the passivation layer thickness should be in the range or lower than that of the phonon wavelength provided in table \ref{tab:PhononWavelength} to improve the thermal dissipation.\\

